Disentangled Graph Social Recommendation

Social recommender systems have drawn a lot of attention in many online web services, because of the incorporation of social information between users in improving recommendation results. Despite the significant progress made by existing solutions, we argue that current methods fall short in two limitations: (1) Existing social-aware recommendation models only consider collaborative similarity between items, how to incorporate item-wise semantic relatedness is less explored in current recommendation paradigms. (2) Current social recommender systems neglect the entanglement of the latent factors over heterogeneous relations (e.g., social connections, user-item interactions). Learning the disentangled representations with relation heterogeneity poses great challenge for social recommendation. In this work, we design a Disentangled Graph Neural Network (DGNN) with the integration of latent memory units, which empowers DGNN to maintain factorized representations for heterogeneous types of user and item connections. Additionally, we devise new memory-augmented message propagation and aggregation schemes under the graph neural architecture, allowing us to recursively distill semantic relatedness into the representations of users and items in a fully automatic manner. Extensive experiments on three benchmark datasets verify the effectiveness of our model by achieving great improvement over state-of-the-art recommendation techniques. The source code is publicly available at: https://github.com/HKUDS/DGNN.

==> fig/hyper_HR_10.tex <==

% \begin{filecontents*}{latdimHR.txt}
% para    Ciao      Epinions      Yelp 
% 4       -20.3083  -9.7501	    -6.2478      
% 8       -11.3690  -3.1954	    -0.7645
% 16      0         0	            0
% 32      -3.7171   -0.7784	    -0.2031
% \end{filecontents*}


\begin{tikzpicture}
\begin{axis}[
    xlabel={Hidden State Size $d$},
    ylabel={HR Decrease(\%)},
    xmin=2,xmax=34,
    ymin=0.4, ymax=0.85,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.2},
    label style={scale=2},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2.2}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {latdimHR.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {latdimHR.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {latdimHR.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{Ciao, Epinions, Yelp};

\end{axis}
\end{tikzpicture}









\begin{tikzpicture}
\begin{axis}[
    xlabel={\# of GNN Layers},
    ylabel={HR Decrease(\%)},
    xmin=-0.2,xmax=3.2,
    ymin=-37,ymax=3,
    xtick={0,1,2,3},
    xticklabels={0,1,2,3},
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.5},
    label style={scale=2},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=3}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {gnnLayersHR.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {gnnLayersHR.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {gnnLayersHR.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{\huge Ciao, \huge Epinions, \huge Yelp};

\end{axis}
\end{tikzpicture}








\begin{tikzpicture}
\begin{axis}[
    xlabel={\# of Memory Units},
    ylabel={HR Decrease(\%)},
    xmin=1,xmax=17,
    ymin=-11.5,ymax=1,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.5},
    label style={scale=2},
    % y label style={at={{axis description cs:0.5,-0.1}},anchor=west},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=3}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {memoryUnitHR.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {memoryUnitHR.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {memoryUnitHR.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{\huge Ciao, \huge Epinions, \huge Yelp};

\end{axis}
\end{tikzpicture}


==> fig/hyper_NDCG_10.tex <==




\begin{tikzpicture}
\begin{axis}[
    xlabel={Hidden State Size $d$},
    ylabel={NDCG Decrease(\%)},
    xmin=2,xmax=34,
    ymin=-25.0, ymax=2,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.5},
    label style={scale=2},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=2.2}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {latdimNDCG.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {latdimNDCG.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {latdimNDCG.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{\huge Ciao, \huge Epinions, \huge Yelp};

\end{axis}
\end{tikzpicture}









\begin{tikzpicture}
\begin{axis}[
    xlabel={\# of GNN Layers},
    ylabel={NDCG Decrease(\%)},
    xmin=-0.2,xmax=3.2,
    ymin=-48,ymax=3,
    xtick={0,1,2,3},
    xticklabels={0,1,2,3},
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.5},
    label style={scale=2},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=3}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {gnnLayersNDCG.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {gnnLayersNDCG.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {gnnLayersNDCG.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{\huge Ciao, \huge Epinions, \huge Yelp};

\end{axis}
\end{tikzpicture}








\begin{tikzpicture}
\begin{axis}[
    xlabel={\# of Memory Units},
    ylabel={NDCG Decrease(\%)},
    xmin=1,xmax=17,
    ymin=-17,ymax=1,
    legend columns=1,
    legend cell align=right,
    grid=both,
    every axis plot/.append style={ultra thick},
    every tick label/.append style={scale=1.5},
    label style={scale=2},
    % y label style={at={{axis description cs:0.5,-0.1}},anchor=west},
    legend style={
        nodes={scale=1.5, transform shape},
        legend image post style={scale=1.5},
        },
    legend style={at={(1,0)},anchor=south east},
    every axis plot post/.append style={
        every mark/.append style={scale=3}
    }
]
\addplot[color={rgb:blue,4;green,2;yellow,1}, mark=o, dashed, mark options={solid}]
table[x=para, y=Ciao] {memoryUnitNDCG.txt};
\addplot[color={rgb:red,4;green,1;yellow,2}, mark=+, dashed, mark options={solid}]
table[x=para, y=Epinions] {memoryUnitNDCG.txt};
\addplot[color={rgb:red,4}, mark=x, dashed, mark options={solid}]
table[x=para, y=Yelp] {memoryUnitNDCG.txt};
% \addplot[color={rgb:red,4}, mark=otimes, dashed, mark options={solid}]
% table[x=para, y=eco_ndcg] {latFactor-buy.txt};
\legend{\huge Ciao, \huge Epinions, \huge Yelp};

\end{axis}
\end{tikzpicture}


==> response.tex <==

\section*{Response to Reviewers}

We really appreciate the constructive comments of all reviewers, and have carefully addressed them in our revision.

\subsection{Response to Reviewer \#1}

% We would like to thank the reviewer for their careful reading and helpful comments. We have revised the manuscript to address the questions raised by the reviewer.

\noindent \textbf{Comment 1}: The advantages of our method in encoding relation heterogeneity with latent factor disentanglement.\\\vspace{-0.15in}

\noindent \textbf{Response}: Thank you for this insightful feedback. While there exist some works on disentangled learning for recommendation, our new recommender system differs from those studies from the following two aspects: i) most of those models are designed to model the homogeneous relations in recommender system, which cannot be easily adaptive to disentangle the diverse factors behind the heterogeneous relationships due to their various semantics. To fill this gap, our disentangled heterogeneous graph memory network is designed to maintain customized factorized representations for relation heterogeneity and distill the relational knowledge in a fully automatic manner, \eg, without the handcrafted meta-path construction based on domain knowledge. ii) The complex dependencies among the encoded latent factors are ignored in most current studies. In contrast, our DHGM method captures the latent factor-wise inter-dependencies with our designed differentiable memory networks under multiple latent representation
spaces. By doing so, the relation-aware latent factors can effective preserve the disentangled heterogeneous semantics. To address this reviewer's comment, we added more discussion in Section II.C of our revised manuscript to further clarify the advantage of our method in encoding relation heterogeneity with latent factor disentanglement compared with existing works. \\\vspace{-0.1in}

\noindent \textbf{Comment 2}: Further clarification of key challenges of disentangling latent factor with relation heterogeneity. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. While having realized the vital role of encoding disentangled relation heterogeneity in recommendation, it is non-trivial due to the following key challenges: i) Learning the disentangled factors with relation heterogeneity brings the challenge of graph neural networks. In our method, we develop a node- and edge-type dependent memory-augmented network to preserve dedicated semantic representations for different types of interactions,
\ie, user-user, item-item and user-item relationships. ii) Capturing the implicit inter-dependencies among different encoded disentangled relation factors. Our framework proposes external memory units with differentiable
embedding propagation scheme to allow our heterogeneous graph neural network to learn the cross-factor inter-dependencies for expressive disentangled representation learning in our recommender system. To address this reviewer's comment, we add further clarification in Section I to emphasize the tackled key challenges. \\\vspace{-0.1in}

\noindent \textbf{Comment 3}: Fixing identified typos. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for the constructive comment. We have fixed the identified typos in page 1 and page 12. The manuscript has been updated accordingly. We also carefully proofread the paper and address other identified typos. \\\vspace{-0.1in}

\subsection{Response to Reviewer \#2}

% We would like to thank the reviewer for their careful reading and helpful comments. We have revised the manuscript to address the questions raised by the reviewer.

% \noindent \textbf{Comment 1}: Further emphasize the motivation of disentangled representation learning in the stated second limitation.\\\vspace{-0.15in}

% \noindent \textbf{Response}: Thanks for this valuable suggestion. To address the reviewer's comment, we further emphasize the motivation of performing factor disentanglement in Section I. While state-of-the-art social recommender systems are proposed to incorporate social influence into the user-item interaction modeling, the fact that diverse connections are driven by complex various latent factors. Specifically, motivated examples are presented from the perspectives of user social relation and user-item interactive relation. i) User’s intent on interacting (\eg, click, or purchase) an item may be influenced by diverse factors due to different item characteristics, such as the brand and color of products,
% director of a movie. The overlook of finer-grained user interest with the factor-level representation learning, may produce suboptimal recommendation results. ii) In real-life social recommendation scenario, users are socially
% connected due to multifaceted motives. \eg, communities with disparate interests, colleagues, or family members. If we represent user-wise influence without the disentanglement of such social polysemy, the learned user preference can
% hard to be reflective of multiple social contexts. Based on the above discussion, investigating the factor disentanglement with relation heterogeneity is very important but unexplored for existing studies. The heterogeneous relations driven by complex latent factors, brings an urge for the model to encode factorized embeddings pertinent to type-specific relation semantics. \\\vspace{-0.1in}

\noindent \textbf{Comment 1}: Directly argue the shortcomings of related disentangled methods in Section I. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this valuable suggestion. To address this reviewer's comment, we add discussion in fifth paragraph to argue the limitations of related disentangled methods in Section I. Specifically, while state-of-the-art recommender systems are proposed to add disentangled representation learning into the user-item interaction modeling, they merely focusing on single type of relation disentanglement, which are limited to incorporate heterogeneous relational semantics into the recommender system. In other words, an important fact in recommendation has been ignored: diverse semantics with relation heterogeneity can be utilized to enhance the user preference learning in recommender system. We need to learn disentangled user/item factorized embeddings with the awareness of heterogeneous relational context for enhancing the representation power of neural recommender systems. \\\vspace{-0.1in}

\noindent \textbf{Comment 2}: Further clarify the limitations of existing disentangled representation learning in Section II.C. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. To address this comment, we have add more discussion in the second paragraph of Section II.C to clarify this point. While there exist some works on disentangled learning for recommendation, our new recommender system differs from those studies from the following two aspects: i) most of those models are designed to model the homogeneous relations in recommender system, which cannot be easily adaptive to disentangle the diverse factors behind the heterogeneous relationships due to their various semantics. To fill this gap, our disentangled heterogeneous graph memory network is designed to maintain customized factorized representations for relation heterogeneity and distill the relational knowledge in a fully automatic manner, \eg, without the handcrafted meta-path construction based on domain knowledge. ii) The complex dependencies among the encoded latent factors are ignored in most current studies. In contrast, our DHGM method captures the latent factor-wise inter-dependencies with our designed differentiable memory networks under multiple latent representation spaces. By doing so, the relation-aware latent factors can effective preserve the disentangled heterogeneous semantics. While one recent work DisenHAN~\cite{wang2020disenhan} attempts to generate disentangled embeddings with heterogeneous context, it still requires domain knowledge to manually construct meta-paths for modeling heterogeneous relations, which can hardly be adaptive to different recommendation tasks. The performance superiority between our method and DisenHAN has been validated in the evaluation.. \\\vspace{-0.1in}

\noindent \textbf{Comment 3}: Further explanation of memory, prototype, $\phi$, $\eta$. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. In our method, Inspired by the strength of memory neural networks in disentangled representation learning, our
DHGM proposes to augment the graph neural network with
differentiable memory components under multiple latent representation
spaces. In our model, each memory unit corresponds to a factor prototype. To capture the heterogeneous characteristic in the knowledge-enhanced social recommendation, we propose to parameterize the relation heterogeneity into vertex- and edge-type dependent embedding projection through external memory units. Here, the learned $\eta$ represents the importance weight of individual factorized embeddings with the awareness of relation type. During the message passing paradigm, $\phi$ denotes the message propagated from the source node to the target node. In our method, customized factor disentanglement is enabled for capturing heterogeneous relational semantics. \\\vspace{-0.1in}

\noindent \textbf{Comment 4}: The relation between our memory neural networks and existing ones. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. In our method, we integrate the memory neural networks with two new dimensions, namely, heterogeneous relation learning and factor disentanglement techniques. In particular, our DHGM generalizes the relation heterogeneity encoding with the maintaining the relation-aware disentangled representations, under the heterogeneous graph memory-augmented message passing. This new model design brings the novelty of memory neural network, which has not been tackled before. \\\vspace{-0.1in}

\noindent \textbf{Comment 5}: Components in our proposed new method to address the limitations of existing works. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this useful suggestion. While having realized the vital role of encoding disentangled relation heterogeneity in recommendation, it is non-trivial due to the following key challenges: i) Learning the disentangled factors with relation heterogeneity brings the challenge of graph neural networks. In our method, we develop a node- and edge-type dependent memory-augmented network to preserve dedicated semantic representations for different types of interactions,
\ie, user-user, item-item and user-item relationships. ii) Capturing the implicit inter-dependencies among different encoded disentangled relation factors. Our framework proposes external memory units with differentiable
embedding propagation scheme to allow our heterogeneous graph neural network to learn the cross-factor inter-dependencies for expressive disentangled representation learning in our recommender system. To address this reviewer's comment, we add further clarification in Section I to emphasize the tackled key challenges. \\\vspace{-0.1in}

\noindent \textbf{Comment 6}: The meaning of $\eta_1$ and $\eta_m$ in Fig. 1. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. $\eta_1$ and $\eta_m$ respectively represents the learned importance weight of the first and $m$-th memory unit corresponding to the encoded factorized embeddings. To address this comment, we update the description of Fig.1 to clarify this point. \\\vspace{-0.1in}

\noindent \textbf{Comment 7}: Difference in item dependency representation learning with previous works. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for pointing out this. Our item dependency representation learning technique differs from previous work by distilling disentangled dependency representations with learning latent factors.  \\\vspace{-0.1in}

\noindent \textbf{Comment 8}: Illustration of three graph layers in Fig.2. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment, in our model figure, we just illustrate the multi-layer graph propagation framework with three graph layers. It is not a fixed design in our model. The experiments in Section V.F (hyperparameter studies) investigate the impact of the number of graph propagation layers in the model performance. We can observe that propagating embeddings across two-hop neighboring nodes brings performance improvement. By stacking more graph layers, the performance will slightly drop due to the over-smoothing problem of graph neural architecture.\\\vspace{-0.1in}

\subsection{Response to Reviewer \#3}

\noindent \textbf{Comment 1}: Discussion of context-aware recommendation.\\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this insightful suggestion. To address this comment, we add a paragraph in the related work section (Section II) to discuss this research line. In particular, There exist some relevant research works focusing in developing context-aware recommender systems with the consideration of various context in different recommendation scenarios [1], [21]. One of such early works is CAMF which extends the conventional matrix factorization framework to incorporate contextual information for rating prediction [4]. From the user dimension, STARS [21] combines the user-wise relations from online social network and the recent user-specific contextual features to enhance collaborative filtering. Kaleido [44] proposes to model uesrs' affective states together with users' interaction records for social recommendation. From the items' content dimension, LBSNs [2] learns the mapping from items' contextual features to users' prefer- ence tags in Point-of-Interest recommendation. CARL [45] proposes to fuse the textual context information of items and the interaction-based embeddings for better representation learning. Additionally, knowledge graphs have also been considered as useful contextual signals to be incorporated into recommender system to improve performance in KGIN [42] and CASR [29]. Compared to the existing context-aware methods, our DHGM better captures the contextual information with our disentangled graph relation learning for both user-side and item-side contexts. \\\vspace{-0.1in}

\noindent \textbf{Comment 2}: Brief description of architecture overview at the beginning of the solution section. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this constructive suggestion. To address this comment, we added brief description of architecture overview at the beginning of Section IV (Methodology). In general, our new method consists of three key components: i) Memory-augmented relation heterogeneity encoder which parameterize
the relation heterogeneity into vertex- and edge-type dependent embedding projection through our designed external memory units under heterogeneous graph neural networks. ii) Disentangled message aggregation with relation heterogeneity that fuses the disentangled relational context from both interactive patterns and side information. iii) Model forecasting stage which incorporates the heterogeneous factorized embeddings into the model optimized objective for recommendation. \\\vspace{-0.1in}

\noindent \textbf{Comment 3}: Test results on Epionions dataset. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. To address this comment, The test results on Epionions dataset have been added in Table III (evaluation varying top-$N$) and Figure.5 (heterogeneous data ablation study). From the added results, the performance superiority of our method compared with state-of-the-art baselines can be observed. This observation is consistent with the results on other datasets, which can further confirms the effectiveness of our DHGM model.\\\vspace{-0.1in}

\noindent \textbf{Comment 4}: Equations and references for the evaluation metrics in Section V.A.3.\\\vspace{-0.15in}

\noindent \textbf{Response}: Thank you so much for your advice. To address reviewer's question, we have updated Section V.A.3 to include the equations and references for the evaluation metrics. We focus on top-$N$ item recommendation and use two widely adopted metrics for evaluation: Hit Rate (HR)@$N$ and Normalized Discounted Cumulative Gain (NDCG)@$N$ with the top-$N$ ranked positions~\cite{chen2018sequential, wang2019neural}, to measure the recommendation accuracy of each evaluated method. Formally, the metrics are calculated as follows:
\begin{align}
HR@N&=\frac{\sum_{i=1}^M\sum_{j=1}^N r_{i,j}}{M}\nonumber\\
NDCG@N&=\sum_{i=1}^M \frac{\sum_{j=1}^N r_{i,j} / \log_2(j+1)}{M\cdot IDCG_i}
\end{align}
where $M$ denotes the number of tested users, $r_{i,j}=1$ if the $j$-th item in the ranked list of the $i$-th user is the positive item, and $r_{i,j}=0$ otherwise. The numerator of NDCG@$N$ is the discounted cumulative gain (DCG)@$N$, and $IDCG_i$ denotes the possible maximum DCG@$N$ value for the $i$-th tested user. \\\vspace{-0.1in}

\noindent \textbf{Comment 5}: The meaning of ``Imp'' in Table II.\\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. In the overall comparison Table II, ``Imp'' represents the relatively performance improvement between our DHGM method and each compared baseline. That's the reason why we not report this for our DHGM. We add clarification in table description for this point in our revision.\\\vspace{-0.1in}

\noindent \textbf{Comment 6}: Redraw the right part of Figure 1 and Figure 3. \\\vspace{-0.15in}

\noindent \textbf{Response}: Thanks for this comment. We redraw the right part of Figure 1 and Figure 3 to make it clear.







